Micro-Vibration Modes Reconstruction Based on Micro-Doppler Coincidence Imaging

Micro-vibration, a ubiquitous nature phenomenon, can be seen as a characteristic feature on the objects, these vibrations always have tiny amplitudes which are much less than the wavelengths of the sensing systems, thus these motions information can only be reflected in the phase item of echo. Normally the conventional radar system can detect these micro vibrations through the time frequency analyzing, but these vibration characteristics can only be reflected by time-frequency spectrum, the spatial distribution of these micro vibrations can not be reconstructed precisely. Ghost imaging (GI), a novel imaging method also known as Coincidence Imaging that originated in the quantum and optical fields, can reconstruct unknown images using computational methods. To reconstruct the spatial distribution of micro vibrations, this paper proposes a new method based on a coincidence imaging system. A detailed model of target micro-vibration is created first, taking into account two categories: discrete and continuous targets. We use the first-order field correlation feature to obtain objective different micro vibration distribution based on the complex target models and time-frequency analysis in this work.

==> photo/backup.tex <==
The ratio of transverse strain to longitudinal strain is known as the Poisson's ratio of solid materials according to the solid material general feature\cite{Contin1}. Generalizing the equation of wave motion to a two-dimensional plane when the turning radius is rectangular section
\begin{equation}
\nabla^{4} w+\frac{3 \rho\left(1-\mu^{2}\right)}{E h^{2}} \frac{\partial^{2} w}{\partial t^{2}}=0
\end{equation}
Where $\nabla^{4}$ is the quadruple-harmonic operator, $E$ is Young modulus of different materials, $\mu$ is its Poisson's ratio, $\rho$ is its intensity, $2h$ is the thickness, and $w$ represents the vibration function in the time-domain. Under the Kirchhoff $G$ model, the target can be considered as a sheet when its thickness is substantially smaller than its surface size. This part establishes the small deflection bending theory of elastic sheets and provides an accurate model of transverse vibration of rectangular plates. For other types of objects, the vibration model is adaptable by modifying the initial conditions and boundary conditions, which will not be classified or discussed in this study. The basic assumptions can be summarized as follow: the middle plane bisecting the plate thickness is the central plane, set central plane as $xOy$ plane, the $Rt$ coordinate space system is established as shown in Fig. 6. When a sheet bends, the central plane becomes a curved surface known as an elastic surface, and the displacement of a random point on this plane is $u$, $v$, and $w$, which correspond to the directions $x$, $y$, and $z$, respectively, where $w$ is the deflection.\\
\begin{enumerate}
\item Normal line hypothesis : The normal line which is perpendicular to the central plane remains straight in the whole procession, and also remains perpendicular to the curved surface of elasticity. In the other way, even though when the transverse shear stresses $\tau_{x z}$ and $\tau_{y z}$ are nonzero, the transverse shear deformation $\gamma_{x z}$ and $\gamma_{y z}$ are ignored.
\item The internal stresses of a bending plate are mainly $\sigma_{x}$, $\sigma_{y}$ and $\tau_{x y}$, and the secondary stresses are $\tau_{x z}$ and $\tau_{y z}$, the minimum stress is $\sigma_z$.
\item The change of thickness should be ignored, i.e. $\varepsilon_{z}=0$, so that every points on the line perpendicular to the elastic plate could have the same transverse  displacement $w$, which indicates that $w$ has no relation with $z$.
\item Deflection $w$ should be much less than the thickness of the sheet $h$, that is to say, all points on the surface of the central plane remain on the central plane during the target deformation.
\end{enumerate}
The rectangle infinitesimals $dxdy$ on the central plane can be replaced by the infinitesimal bodies $hdxdy$ based on the hypotheses listed above , so that the differential equation of the sheet's transverse vibration can be written as
\begin{equation}
D_{0} \nabla^{4} w+\rho h \frac{\partial^{2} w}{\partial t^{2}}=p(x, y, t)
\end{equation}
where $p(x,y,t)$ is a stress function, which represents the forced vibration on the target sheet, and $D_{0}=\frac{E h^{3}}{12\left(1-\mu^{2}\right)}$ is the flexural rigidity of the sheet, the equation should be transformed to a tensor form if the infinitesimal has not been replaced by rectangle infinitesimals,
\begin{equation}
\boldsymbol{\sigma}=\left(\begin{array}{l}
\sigma_{x} \\
\sigma_{y} \\
\tau_{x y}
\end{array}\right), \boldsymbol{D_1}=\left(\begin{array}{ccc}
1 & \mu & 0 \\
\mu & 1 & 0 \\
0 & 0 & \frac{1-\mu}{2}
\end{array}\right)
\end{equation}where $D_0$ represents scalar and $D_1$ represents non-scalar. Equation $(35)$ can be further organized as
\begin{equation}
\boldsymbol{\sigma}=\frac{E}{1-\mu^{2}} \boldsymbol{D_1} \varepsilon=\frac{E z}{1-\mu^{2}} \boldsymbol{D_1} \boldsymbol{\kappa}
\end{equation}where $\kappa$ is the transverse strain vector, thus the torque tensor can be determined as follow
\begin{equation}
\boldsymbol{M}=\frac{E}{1-\mu^{2}} \boldsymbol{D_1} \boldsymbol{\kappa} \int_{h / 2}^{-h / 2} z^{2} d z
\end{equation}Simplifying boundary conditions, the boundary of the sheet has no deflection and no bending moment $(x=0)$, thus we could assume that boundary conditions can be set as follow,
\begin{equation}
\left.w\right|_{x=0}=0,\left.\frac{\partial w}{\partial x}\right|_{x=0}=0
\end{equation}Assuming that all vibrations composed by the forced vibrations can be seen as a linear superposition of free vibrations, thus we can discuss the free vibration of sheets first, when $p(x, y, t)=0$, the free vibration function can be acquired
\begin{equation}
D_{0} \nabla^{4} w+\rho h \frac{\partial^{2} w}{\partial t^{2}}=0
\end{equation}
The vibration function should have a formal solution of separation of variables,
\begin{equation}
w(x, y, t)=W(x, y) \sin (\omega t+\phi)
\end{equation}
where $W(x,y)$ is the principal mode, so $\omega$ is the corresponding characteristic frequency. Subtitling equation $(40)$ into equation $(39)$,
\begin{equation}
\nabla^{4} W-\beta^{4} W=0
\end{equation}
where $\beta^{4}=\frac{\rho h}{D_{0}} \omega^{2}$, and because of the homogeneity of the boundary conditions for $W$, $\omega$ can be rewritten as $W$ directly. For the case of four-sided supporting, the exact principal mode vibration expression can be obtained as ,
\begin{equation}
W_{i, j}(x, y)=A_{i, j} \sin \frac{i \pi x}{a} \sin \frac{j \pi y}{b}, i, j=1,2,3, \ldots
\end{equation}
where $A_{i j}$ is the amplitude corresponding to different order vibration. From equation $(42)$ we can know that if we need the final form of principal mode, we need to solve the differential equation $(41)$, and $\beta$ should satisfy the boundary condition
\begin{equation}
\left[\left(\frac{i \pi}{a}\right)^{2}+\left(\frac{j \pi}{b}\right)^{2}\right]^{2}-\beta^{4}=0
\end{equation}
which can be rewritten as the form of eigenfrequency,
\begin{equation}
\omega_{i, j}=\pi^{2}\left(\frac{i^{2}}{a^{2}}+\frac{j^{2}}{b^{2}}\right)
\end{equation}
The precise orthogonality of eigenfrequency among the primary vibration can guarantee the decomposition is regular. However, our method of detection focus on the whole plane, we only need the variations form of the differential equation on the whole sheet plane$(\Omega)$ :
\begin{equation}
\iint_{\Omega}\left(D_{0} \nabla^{4} W-\omega^{2} \rho h W\right) \delta W d x d y=0
\end{equation}The functional characteristic values of plate vibrations can also be obtained:
\begin{equation}
\omega^{2}=\frac{\iint_{\Omega} D_{0} \boldsymbol{\kappa}^{T} \boldsymbol{D_1} \boldsymbol{\kappa} d x d y}{\iint_{\Omega} \rho h W^{2} d x d y}
\end{equation}
The principal modes $W_i(x,y)$ and $W_j(x,y)$ have two different natural frequencies $\omega_i$ and $\omega_j$ under the condition of linear indexes, thus $W$ can be written as
\begin{equation}
W=a_{i} W_{i}+a_{j} W_{j}
\end{equation}
where $a_i$ and $a_j$ are the constant coefficients of each components respectively, considering $\kappa$ is a linear tensor, the relationship between $W_i$, $W_j$ and $\kappa$ can be written as,
\begin{equation}
\boldsymbol{\kappa}(W)=a_{i} \boldsymbol{\kappa}\left(W_{i}\right)+a_{j} \boldsymbol{\kappa}\left(W_{j}\right)
\end{equation}
Substituting equations $(47)$ and $(48)$ into $(46)$, we can obtain
\begin{equation}
\begin{aligned}
&\iint_{\Omega} D_{0} \boldsymbol{\kappa}^{T} \boldsymbol{D_1} \boldsymbol{\kappa} d x d y \\
&=\iint_{\Omega} D_{0}\left[a_{i} \boldsymbol{\kappa}\left(W_{i}\right)+a_{j} \boldsymbol{\kappa}\left(W_{j}\right)\right]^{T} \\
&\quad \times \boldsymbol{D_1}\left[a_{i} \boldsymbol{\kappa}\left(W_{i}\right)+a_{j} \boldsymbol{\kappa}\left(W_{j}\right)\right] d x d y \\
&=a_{i}^{2} k_{i i}+a_{i} a_{j} k_{i j}+a_{j} a_{i} k_{j i}+a_{j}^{2} k_{j j}
\end{aligned}
\end{equation}and
\begin{equation}
\begin{aligned}
&\iint_{\Omega} \rho h W^{2} d x d y \\
&=\iint_{\Omega} \rho h\left(a_{i} W_{i}+a_{j} W_{j}\right)\left(a_{i} W_{i}+a_{j} W_{j}\right) d x d y \\
&=a_{i}^{2} m_{i i}+a_{i} a_{j} m_{i j}+a_{j} a_{i} m_{j i}+a_{j}^{2} m_{j j}
\end{aligned}
\end{equation}
The constants in equations $(49)$ and $(50)$ satisfy,
\begin{equation}
\begin{aligned}
&k_{m n}=k_{n m}=\iint_{\Omega} D_{0} \boldsymbol{\kappa}^{T}\left(W_{m}\right) \boldsymbol{D_1} \boldsymbol{\kappa}\left(W_{n}\right) d x d y \\
&m_{m n}=m_{n m}=\iint_{\Omega} \rho h W_{m} W_{n} d x d y
\end{aligned}
\end{equation}If the matrices $\boldsymbol{K}$,$\boldsymbol{M}$ and the vector $\boldsymbol{a}$ are
\begin{equation}
\boldsymbol{K}=\left[\begin{array}{ll}
k_{i i} & k_{i j} \\
k_{j i} & k_{j j}
\end{array}\right], \boldsymbol{M}=\left[\begin{array}{ll}
m_{i i} & m_{i j} \\
m_{j i} & m_{j j}
\end{array}\right], \boldsymbol{a}=\left[\begin{array}{l}
a_{i} \\
a_{j}
\end{array}\right]
\end{equation}
the characteristic value function $(46)$ can be conveniently given by the quadratic form of the vector,
\begin{equation}
\omega^{2}=\frac{\boldsymbol{a}^{T} \boldsymbol{K}\boldsymbol{a}}{\boldsymbol{a}^{T} \boldsymbol{M} \boldsymbol{a}}
\end{equation}
The vector $\boldsymbol{a}$ can be seen as a variable in equation $(53)$, when the derivative of the characteristic value function is zero
\begin{equation}
\delta\left(\omega^{2}\right)=0
\end{equation}
then we can have
\begin{equation}
\frac{1}{\left(\boldsymbol{a}^{T} \boldsymbol{M} \boldsymbol{a}\right)^{2}}\left[\left(\boldsymbol{a}^{T} \boldsymbol{M}  \boldsymbol{a}\right) \delta\left(\boldsymbol{a}^{T} \boldsymbol{K}  \boldsymbol{a}\right)-\left(\boldsymbol{a}^{T} \boldsymbol{K}  \boldsymbol{a}\right) \delta\left(\boldsymbol{a}^{T} \boldsymbol{M}  \boldsymbol{a}\right)\right]=0
\end{equation}
Consequently, equation $(55)$ can be simplified on the based of equation $(53)$
\begin{equation}
\delta^{T}(\boldsymbol{a})\left(\boldsymbol{K}-\boldsymbol{\omega}^{2}\boldsymbol{M} \right) \boldsymbol{a}=0
\end{equation}
According to the arbitrary of $\delta^{T}(\alpha)$, 
\begin{equation}
\left(\boldsymbol{K}-\boldsymbol{\omega}^{2}\boldsymbol{M} \right) \boldsymbol{a}=0
\end{equation}
Assigning $a_i=0,a_j=1$ and $a_j=0,a_i=1$ respectively, the difference is 
\begin{equation}
\left(\omega_{i}^{2}-\omega_{j}^{2}\right) m_{i j}=0
\end{equation}
if $\omega_{i}^{2} \neq \omega_{j}^{2}$, then $m_{i j}=\delta_{i j}$. For the same, $k_{i j}=\delta_{i j}$. When the characteristic value equation gives multiple roots, we can also make the $n$th multiple roots give $n$th orthogonal principal modes through reasonable orthogonalization.  Thus the orthogonality among cross-indexes principal modes can be given as
\begin{equation}
\begin{aligned}
&\iint_{\Omega} D_{0} \kappa^{T}\left(W_{i j}\right) D_{1} \kappa\left(W_{m n}\right) d x d y=\omega_{m n}^{2} \delta_{i m} \delta_{j n} \\
&\iint_{\Omega} \rho h W_{i j} W_{m n} d x d y=\delta_{i m} \delta_{j n}
\end{aligned}
\end{equation}
The forced vibration of rectangular sheet can be determined by the oscillator composition after we have the orthogonality among the principal modes on the surface of rectangular sheet. Expanding $w$ to bi-series as orthogonal principal modes
\begin{equation}
w(x, y, t)=\sum_{i=1}^{\infty} \sum_{j=1}^{\infty} W_{i j}(x, y) \eta_{i j}(t)
\end{equation}
Subtitling equation $(34)$,
\begin{equation}
\begin{aligned}
&D_{0} \sum_{i=1}^{\infty} \sum_{j=1}^{\infty}\left[\nabla^{4} W_{i j}(x, y)\right] \eta_{i j}(t) \\ 
& +\rho h \sum_{i=1}^{\infty} \sum_{j=1}^{\infty} W_{i j}(x, y) \ddot{\eta}_{i j}(t)=p(x, y, t)
\end{aligned}
\end{equation}
Multiplying with $W_{m n}(x,y)$ on both sides of equation $(61)$ and integrating $x$ and $y$ over $\Omega$,
\begin{equation}
\begin{aligned}
& \sum_{i=1}^{\infty} \sum_{j=1}^{\infty} \eta_{i j}(t) \iint_{\Omega} D_{0}\left[\nabla^{4} W_{i j}(x, y)\right] W_{m n}(x, y) \mathrm{d} x \mathrm{~d} y \\
& +\sum_{i=1}^{\infty} \sum_{j=1}^{\infty} \ddot{\eta}_{i j}(t) \iint_{\Omega} \rho h W_{i j}(x, y) W_{m n}(x, y) \mathrm{d} x \mathrm{~d} y \\
&= \iint_{\Omega} p(x, y, t) W_{m n}(x, y) \mathrm{d} x \mathrm{~d} y
\end{aligned}
\end{equation}
Then the canonical equation can be acquired by using conditions of orthogonality,
\begin{equation}
\begin{aligned}
& \ddot{\eta}_{m n}(t)+\omega_{m n}^{2} \eta_{m n}(t)=q_{m n}(t) \\ 
 \quad & q_{m n}(t)=\iint_{\Omega} p(x, y, t) W_{m n}(x, y) \mathrm{d} x \mathrm{~d} y
\end{aligned}
\end{equation}
When the sheet satisfy the initial condition
\begin{equation}
w(x, y, 0)=\lambda_{1}(x, y),\left.\quad \frac{\partial w}{\partial t}\right|_{t=0}=\lambda_{2}(x, y)
\end{equation}
then we can determine the initial condition in canonical coordinate
\begin{equation}
\begin{aligned}
&\eta_{m n}(0)=\iint_{\Omega} \rho h \lambda_{1}(x, y) W_{m n}(x, y) \mathrm{d} x \mathrm{~d} y \\
&\dot{\eta}_{m n}(0)=\iint \rho h \lambda_{2}(x, y) W_{m n}(x, y) \mathrm{d} x \mathrm{~d} y
\end{aligned}
\end{equation}
The solution of equation $(63)$ should be
\begin{equation}
\begin{aligned}
\eta_{m n}(t)&= \eta_{m n}(0) \cos \omega_{m n} t+\frac{\dot{\eta}_{m n}(0)}{\omega_{m n}} \sin \omega_{m n} t \\
&+\frac{1}{\omega_{m n}} \int_{0}^{t} q_{m n}(\tau) \sin \omega_{m n}(t-\tau) \mathrm{d} \tau
\end{aligned}
\end{equation}





\section{Conventional micro-vibration extraction methods by time-frequency spectrum analysis}
The frequency modulated chirped signal is used to detect target micro-vibration in existing GI systems. Following coherence with the $LO$ signal, the desired micro-vibration characteristics can be detected using time-frequency processing methods \cite{PL1}, such as the short time Fourier transform ($STFT$). Given that multiple time-frequency characteristic curves overlap in the time-frequency spectrum in most scenes, and these overlaps may cause aliasing in a specific target recognition, it is necessary to investigate the algorithms for extracting these characteristic curves from the time frequency spectrum. For a certain vibration mode which awaits to be extracted from the other vibration modes and background noise, the time-frequency curves extraction algorithms are necessary for curves extraction. There are existing curves extraction algorithms\cite{TF2}, such as curve tracking algorithm or the predictive algorithm using particle filter\cite{TF1}.
Nearly all of these algorithms will lost the correlation with the original target energy fluctuation, whereas the energy fluctuation integrity of the target is important for the correlation processing for the first-order field correlation method. The signal lost its energy fluctuation integrity means it lost its relevancy with the reference patterns. In this part, the theoretical derivation of the time-frequency analysis technique is presented, and the limitations of the time-frequency approaches are analyzed using the theoretical target model.\\ 
The continuous target can be seen as an assemble of scattering points which have constraint of spatial transverse propagation, the continuous target model is a special case of the discrete target models namely. Set the discrete target detecting scenario as an example, substituting the discrete target model given in equation $(32)$ into electronic signal $i(t)$ which is output from the coherence detector as shown in equation $(28)$
\begin{equation}
\begin{aligned}
i(t) &=\sum_{k=1}^{K} \sum_{n=0}^{\infty} P\left(x_{o, k}, t\right) \exp \left(\phi_{0}\right) \mathcal{T}\left(x_{o, k}\right) \\
& \times \exp(j k_{\lambda} f_{I F} t) \exp \left[j 2 k_{\lambda} z_{k, n} \cos \left(2 \pi f_{k, n} t+\phi_{k, n}\right)\right]
\end{aligned}
\end{equation}
where $\exp \left(\phi_{0}\right)$ is a constant phase item produced by the Fresnel diffraction of transmitting radiation field, which can be expanded explicitly,

\begin{equation}
\exp \left(\phi_{0}\right)=\exp \left(\frac{j 4 \pi}{\lambda_{c}}z_{0}\right) \exp[\frac{j k_{\lambda}}{2z_2}(x_r - x_o)^2]
\end{equation}

An echo phase item consists of the $k$th scattering points harmonic vibration linear superposition according to the electronic scattering theory. When analyzing the time domain characteristics of a vibration micro-Doppler signal, the first kind of m-order Bessel function can be used to expand equation $(69)$
\begin{equation}
\begin{aligned}
i(t) &=\sum_{k=1}^{K} P\left(x_{o, k}, t\right) \exp \left(\phi_{0}\right) \mathcal{T}\left(x_{o, k}\right)   \\
& \times \sum_{n = 0}^{\infty} \sum_{m=-\infty}^{\infty}  J_{m}(B) \exp \left[j 2 \pi (f_{I F} + m f_{k,n} t)\right]
\end{aligned}
\end{equation}where, $f_{k,n}$ is the micro-Doppler frequency caused by vibrations, and $J_m(B)$ stands for the $m$-order Bessel function that can be written in details, and $B$ is the parameter of the Bessel function, its expression is
\begin{equation}
J_{m}(B)=\frac{1}{2 \pi} \int_{-\pi}^{\pi} \exp [j(B \sin u-m u)] d u
\end{equation}
As a consequence of the time-frequency analysis, the desired time-frequency characteristics curves could well be shown. Many advanced mathematical analysis methods of time-frequency characteristic curves exist, however they will not be discussed in depth in this study. Smooth-pseudo Wigner-ville Distribution as shown in Fig .7 is an analyzing method which remains high resolution in both time domain and frequency domain. It is an appropriate method to precisely extract and analyze time-frequency characteristics of signals.
The primary goal of these approaches is to separate time and frequency characteristics; the basic model of time-frequency curves can be expressed as $(71)$ regardless of system configurations or time-frequency resolution
\begin{equation}
\begin{aligned}
I(f,t) &=\sum_{k=1}^{K} \sum_{n = 0}^{\infty} \sum_{m=-\infty}^{\infty}  P\left(x_{o, k}, t\right) \exp \left(\phi_{0}\right) \mathcal{T}\left(x_{o, k}\right)  \\
& \times \exp \left(-j m \phi_{k,n}\right) J_{m}\left(4 \pi z_{k,n} / \lambda\right) \\
&\times\delta\left[f-f_{I F}-m f_{k,n}(t)\right]
\end{aligned}
\end{equation}

\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth,height=0.5\linewidth]{pdf/filteredcurve.pdf}
\caption{The SPWVD result of two random time-frequency curves which has different initial phases, amplitudes and vibration frequencies. In the majority of physical scenarios, the time-frequency curves would occur aliasing in time-frequency spectrum as shown in this figure.}
\label{fig：1}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth,height=0.7\linewidth]{pdf/twosignals.pdf}
\caption{(a) shows the result of the extracting curves from the spectrum shown in Fig. 7, and the extracting algorithm used in this scenario is curve tracking algorithm. (b) shows the result of the original characteristic curve as a comparison, both of them are processed with the same noise-filtered procession   }
\label{fig：1}
\end{figure}
The Dirac function in equation $(73)$ shows that the frequency spectrum is composed by a series of  frequency peaks at the center of $f_{IF}$ and side lobes in the interval of $f_{k,n}$. Each main frequency peak $f_{IF}$ has its own broaden $ J_{m}\left(4 \pi z_{k,n} / \lambda\right)$. The time-frequency spectrum that illustrates the time frequency characteristic curves is obtained using the short-time Fourier transform $(STFT)$. Making the window function time scale $u$ the same as the single pulse lasting time $(u=T)$ so that the speckle distribution on the object surface could remain stable in a single time window. Then the translations and micro-vibrations information of objects can be extracted from the time-frequency spectrum. According to the three elements of targets movement (speed, acceleration and the rate action factor of acceleration), the target translation item can be written as,

\begin{equation}
R_{0}=r_{0}+v_{0} u+v_{0}^{\prime} u+v_{0}^{\prime \prime} u
\end{equation}where, $r_0$ is the initial position of target. The time window correlated function $f_D(u)$ can be shown as below,
\begin{equation}
f_{D}(u)=\frac{B}{c T}\left(r_{0}+v_{0} u+v_{0}^{\prime} u+v_{0}^{\prime \prime} u\right)
\end{equation}
and $f_{k,n}$ can also be written as,
\begin{equation}
f_{k,n}(u)=\sum_{n = 0}^{\infty} 2 k_{\lambda} z_{k,n} \cos \left[\frac{2 \pi}{T}\left(u-T\left[\frac{u}{T}\right]\right)\right]
\end{equation}
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth,height=0.7\linewidth]{pdf/energyfluctuations.pdf}
\caption{The two normalized energy fluctuation curves of the two objects illustrated in Fig.7. The extraction method used in this scenario is curves tracking algorithm. The blue curve shows the original target energy fluctuation in the echo and the orange curve shows the extracted target energy fluctuation from the time-frequency spectrum. Since two curves lost their relevancy on energy fluctuation apparently, it is bound to be unsatisfactory for the image reconstructed by correlation algorithms.}
\label{fig：1}
\end{figure}

Thus, if different time-frequency curves are completely independent, there is no overlap between different characteristic curves, the signal energy fluctuations corresponding to different vibrating targets can be separated completely. But in normal situations, characteristic curves always have overlap, and almost all of the targets characteristic curves extracted by the existing algorithms lost energy linearity in pulses to some extent. Even though there are only two curves in the spectrum, as shown in Fig. 8, using the existing curve tracking algorithm to extract a specific curve from the time-frequency spectrum shown in Fig. 7, the curves correlation tracking result is still not satisfactory, especially in the cross items of two curves. Because the exact radiation field energy fluctuation of the target cannot be collected during the extraction procedures, as illustrated in Fig. 9, the reconstruction of imaging cannot be synchronized with the radiation field energy fluctuation during coherent detection.
